Determination of the sign of the decay width difference in the B_s system

The interference between the K+K- S-wave and P-wave amplitudes in B_s -> J/psi K+K- decays with the K+K- pairs in the region around the phi(1020) resonance is used to determine the variation of the difference of the strong phase between these amplitudes as a function of K+K- invariant mass. Combined with the results from our CP asymmetry measurements in B_s -> J/psi phi decays, we conclude that the B_s mass eigenstate that is almost CP =+1 is lighter and decays faster than the mass eigenstate that is almost CP =-1. This determines the sign of the decay width difference DeltaGamma_s == Gamma_L -Gamma_H to be positive. Our result also resolves the ambiguity in the past measurements of the CP violating phase phi_s to be close to zero rather than pi. These conclusions are in agreement with the Standard Model expectations.

==> answerRefereePRL <==
Replies to Referee B:

1) Introduction section: It would be nice to show the relation of two
mass eigenstate and phi_s with the formula so that readers can easily
understand phi_s = 0 gives B_L (light mass eigenstates) to be CP=+1
and phi = pi gives B_L to be CP = -1, or cite Ref.

A: We have added a reference  arXiv:hep-ph/0012219 which discusses 
the relation between mass eigenstate and CP eigenstate in terms of 
phi_s in equation 18. 

2) It would be easier for general readers to understand if explicit
Breit-Wigner formula is given (in footnote-like Ref. ?).

A:  We avoid giving explicit Breit-Wigner formula since no such formula 
is used in the analysis and the explicit  form is model dependent. The method 
itself has been clearly described in ref[5] ([6]  of the new version).


3) Although using sWeight and sFit technique simplifies the fitting,
the technique is rather specialized and not easy to understand for
general readers. It would be more straightforward to readers to extend
the method used in Ref.[3]. Is it essential to use sWeight and sFit
technique in this analysis?

A: While the definition of sWeight involves some cumbersome mathematics,  
the sFit technique is quite simple: it  uses  sWeights to cancel background 
contribution to the likelihood  function and can be  understood as a smart 
way of sideband subtraction. The sFit method  has been clearly described in 
ref [11]. The motivation to use the sFit method  rather than the method in ref [3] 
is because the wider m_KK mass range  leads to higher background level which can be 
better treated using the sFit method  than the method in ref [3]. We believe the use of 
sFit method  is well justified.  Actually the sFit method was already used and  
briefly discussed  in ref [3] for systematics evaluation by comparing the fit 
results using the sFit method and the classic fit method.

4) p 1, left, bottom par (p 1 is defined as Abstract page): In
Ref.[3], it does not seem to be explicitly mentioned that CP-even
final state has larger width than CP-odd state. It can be only seen in
Fig.2 of Ref.[3]. It may be kind to readers if some footnote-like
comments are added about it.

A:  These sentences are rewritten. Fig. 2 of Ref [3] is mentioned. 


5) The number of background events in Table I is in the m_J/psiKK
region of [5200, 5550] MeV ? It is better to be explicitly mentioned.

A:  We have added  "the m_JpsiKK range of 5200-5550 MeV" in the caption of table I.

6) In Table I, "W_p;k, statistical power per signal event" is not
clear. It is also mentioned later in the text (p 3, l, top par.), but
it does not add much information. It is an average value of
Ws(m_J/psiKK) of the candidate events ? In the simultaneous fit,
even-by-event weight Ws(m_J/psiKK) is used ? But, the text implies
that the constant value W_p;k is used. This point should be clarified.

A: W_p;k is a constant for bin k. It is NOT the average value of the sWeights Ws(M_JpsiKK). 
As the first equation of the paper  clearly shows,  in the simultaneous  fit, the log  of 
the PDF value of each candidate is multiplied by two weights: the event-by-evnet  
sWeight Ws(M_JpsiKK) for background subtraction; the bin-by-bin factor W_p;k for 
getting correct error estimates. The factor W_p;k has a value between 0 and 1, which 
depends on the background level in bin k. Without this factor, the Minuit  fit errors will 
be under-estimated.   Empirically the factor W_p;k required to get correct errors  is  
well approximated by the sum of square of Ws(m_JpsiKK) divided by sum of  Ws(m_JpsiKK) 
over all candidates in bin k, which gives the values in the last column of table I. 
Since the technical details are not essential for understanding the physics discussed in 
the paper, we only briefly explain the meaning of W_p;k by saying 
"account for loss of statistical precision in parameter estimation due to background dilution".

7) p 2, right, bottom par: "\delta_S\perp;k" is better to be
explicitly defined like "\delta_s\perp;k = \delta_S - \delta_\perp".
Actually, the definition seems to be "\delta_S - \delta_\perp - pi"
comparing this result with that of Ref.[3].

A: The difference of pi was due to  different  angle conventions used in this paper and Ref [3]. 
We have changed Table II and Fig4 to use the same convention as in Ref [3]. So there is no need 
to add pi in the definition of  the  phase difference  between S-wave and perpendicular P-wave amplitudes, 
denoted  as \delta_S\perp.   We avoid using  symbols \delta_S and \delta_\perp, which are not defined in this paper, 
since only the phase difference is well defined and meaningful. 

8) In the fit, all the events of M_J/psiKK in [5200, 5500] are used ?
or M_J/psiKK is limited to tighter signal region ? It is better to be
mentioned in the text.

A: All the events in 5200-5550 MeV are used. This gives a wide sideband 
for background subtraction using sFit technique.  This is now explicitly mentioned.

9) In Ref.[3], fraction of S-wave component is 0.042 in +-12 MeV
around phi mass, while in Table II, those in corresponding regions are
0.061 and 0.044 which suggests that the fraction is ~0.053 for
combined region (+-12 MeV). For delta_s\perp, Ref.[3] gives 0.03 - pi
= -3.11, while Table II gives ~(-2.92-3.25)/2 ~ -3.08. This difference
is due to the due to the different methods (i.e. effect of sFit) ? If
so, this effect is included in systematic error ?

A:  About half of these differences are due to different methods 
(sFit vs classic fit). Ref. [3]  takes the difference between sFit and 
classic fit results as source of systematics. In this analysis we do not need  
to do so since the use of sFit method should only reduce background related 
systematic effects. Another reason for the differences is the different binning. 
In ref [3], the  +/- 12MeV mass region around phi(1020) is treated as a single bin 
while in this analysis it is divided into two equal bins. This causes some numerical  
changes. Part of the changes can be systematic since we ignore the variation of 
Fs and \delta_S\perp with m_KK in each bin. In the second last paragraph, the systematic 
effect of ignoring this variation on the significance of the negative trend of \delta_S\perp 
vs M_KK is evaluated. 


10) In Fig.1, horizontal bars for region 1 should be extended to 988
MeV (new 998 Mev)?

A: This is fixed.

11) p 3, l, bottom par.: I would suggest to modify "the fraction of
S-wave .... amplitudes " to "F_S;k and \delta_S\perp;k". [ They are
already defined previously. ]

A: This is modified as suggested.

12) p 3, r, bottom par.: Since the Solution II is mirror image of the
Solution I w.r.t -pi/2, the slope of Solution II should be just
opposite sign value (including errors) of Solution I. Therefore, I
would suggest to make it clear as "... for solution I and the opposite
sign for solution II".

A: This is modified as suggested.

13) Ref.[1] and [3] have been published in journals as authors know.

A: This is modified as suggested.

14) Ref.[11]: I could not find arXiv:0905.0724. It may be a typo?

A:  The sFit reference ([11] in old version and [12] in new version) 
can be found on arXiv website  http://arxiv.org/abs/0905.0724 











==> bibliography.tex <==
% $Id: bibliography.tex 9804 2011-09-22 13:39:57Z uegede $
% ===============================================================================
% Purpose: sample file with definition of references
% Author: 
% Created on: 2010-09-24
% ===============================================================================

\clearpage

% Here we include an example of references using plain LaTeX.
%D
%D template development note: references
%D            add more items to cover all usual cases for references?
%D            have references_bibtex.tex template to be used as alternative?
%D

\begin{thebibliography}{99}

\bibitem{Alves:2008zz}
{\bf LHCb Collaboration} Collaboration, A.~Alves {\em et.~al.}, {\it {The LHCb
  Detector at the LHC}},  {\em JINST} {\bf 3} (2008) S08005.

\bibitem{Sjostrand:2006za}
T.~Sjostrand, S.~Mrenna, and P.~Z. Skands, {\it {PYTHIA 6.4 Physics and
  Manual}},  {\em JHEP} {\bf 0605} (2006) 026,
  [\href{http://xxx.lanl.gov/abs/hep-ph/0603175}{{\tt hep-ph/0603175}}].

\bibitem{Skands:2009zm}
P.~Z. Skands, {\it {The Perugia Tunes}},
  \href{http://xxx.lanl.gov/abs/0905.3418}{{\tt arXiv:0905.3418}}.

\bibitem{FerroLuzzi:2005em}
M.~Ferro-Luzzi, {\it {Proposal for an absolute luminosity determination in
  colliding beam experiments using vertex detection of beam-gas interactions}},
   {\em Nucl.Instrum.Meth.} {\bf A553} (2005) 388--399.

\end{thebibliography}



==> lhcb-symbols-def.tex <==
% $Id: lhcb-symbols-def.tex 11862 2011-11-18 17:16:08Z xieyu $
% ===============================================================================
% Purpose: standard LHCb aliases
% Author: Ulrik Egede (adopted by Tomasz)
% Created on: 2009-09-24
% ===============================================================================


% this has to go before \begin{document}
%\usepackage{ifthen} 
%\newboolean{uprightparticles}
%\setboolean{uprightparticles}{true} %Set to false to get italic particle symbols


%%%%% UE 31/3/10

\newcommand{\BAR}[1]{\overline{#1}}


% Experiments
\def\lhcb {LHCb\xspace}
\def\atlas {ATLAS\xspace}
\def\cms {CMS\xspace}
%\def\babar{\mbox{\slshape B\kern-0.1em{\small A}\kern-0.1em B\kern-0.1em{\small A\kern-0.2em R}}}
\def\babar {BABAR\xspace}
\def\belle {BELLE\xspace}
\def\lhc {LHC\xspace}

\ifthenelse{\boolean{uprightparticles}}%
{\def\Palpha      {\ensuremath{\upalpha}\xspace}
 \def\Pbeta       {\ensuremath{\upbeta}\xspace}
 \def\Pgamma      {\ensuremath{\upgamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\updelta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\upepsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\upvarepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\upzeta}\xspace}                 
 \def\Peta        {\ensuremath{\upeta}\xspace}                 
 \def\Ptheta      {\ensuremath{\uptheta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\upvartheta}\xspace}                 
 \def\Piota       {\ensuremath{\upiota}\xspace}                 
 \def\Pkappa      {\ensuremath{\upkappa}\xspace}                 
 \def\Plambda     {\ensuremath{\uplambda}\xspace}                 
 \def\Pmu         {\ensuremath{\upmu}\xspace}                 
 \def\Pnu         {\ensuremath{\upnu}\xspace}                 
 \def\Pxi         {\ensuremath{\upxi}\xspace}                 
 \def\Ppi         {\ensuremath{\uppi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\upvarpi}\xspace}                 
 \def\Prho        {\ensuremath{\uprho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\upvarrho}\xspace}                 
 \def\Ptau        {\ensuremath{\uptau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upupsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\upphi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\upvarphi}\xspace}                 
 \def\Pchi        {\ensuremath{\upchi}\xspace}                 
 \def\Ppsi        {\ensuremath{\uppsi}\xspace}                 
 \def\Pomega      {\ensuremath{\upomega}\xspace}                 

 \def\PDelta      {\ensuremath{\Delta}\xspace}                 
 \def\PXi      {\ensuremath{\Xi}\xspace}                 
 \def\PLambda      {\ensuremath{\Lambda}\xspace}                 
 \def\PSigma      {\ensuremath{\Sigma}\xspace}                 
 \def\POmega      {\ensuremath{\Omega}\xspace}                 
 \def\PUpsilon      {\ensuremath{\Upsilon}\xspace}                 
 
 %\mathchardef\Deltares="7101
 %\mathchardef\Xi="7104
 %\mathchardef\Lambda="7103
 %\mathchardef\Sigma="7106
 %\mathchardef\Omega="710A


 \def\PA      {\ensuremath{\mathrm{A}}\xspace}                 
 \def\PB      {\ensuremath{\mathrm{B}}\xspace}                 
 \def\PC      {\ensuremath{\mathrm{C}}\xspace}                 
 \def\PD      {\ensuremath{\mathrm{D}}\xspace}                 
 \def\PE      {\ensuremath{\mathrm{E}}\xspace}                 
 \def\PF      {\ensuremath{\mathrm{F}}\xspace}                 
 \def\PG      {\ensuremath{\mathrm{G}}\xspace}                 
 \def\PH      {\ensuremath{\mathrm{H}}\xspace}                 
 \def\PI      {\ensuremath{\mathrm{I}}\xspace}                 
 \def\PJ      {\ensuremath{\mathrm{J}}\xspace}                 
 \def\PK      {\ensuremath{\mathrm{K}}\xspace}                 
 \def\PL      {\ensuremath{\mathrm{L}}\xspace}                 
 \def\PM      {\ensuremath{\mathrm{M}}\xspace}                 
 \def\PN      {\ensuremath{\mathrm{N}}\xspace}                 
 \def\PO      {\ensuremath{\mathrm{O}}\xspace}                 
 \def\PP      {\ensuremath{\mathrm{P}}\xspace}                 
 \def\PQ      {\ensuremath{\mathrm{Q}}\xspace}                 
 \def\PR      {\ensuremath{\mathrm{R}}\xspace}                 
 \def\PS      {\ensuremath{\mathrm{S}}\xspace}                 
 \def\PT      {\ensuremath{\mathrm{T}}\xspace}                 
 \def\PU      {\ensuremath{\mathrm{U}}\xspace}                 
 \def\PV      {\ensuremath{\mathrm{V}}\xspace}                 
 \def\PW      {\ensuremath{\mathrm{W}}\xspace}                 
 \def\PX      {\ensuremath{\mathrm{X}}\xspace}                 
 \def\PY      {\ensuremath{\mathrm{Y}}\xspace}                 
 \def\PZ      {\ensuremath{\mathrm{Z}}\xspace}                 
 \def\Pa      {\ensuremath{\mathrm{a}}\xspace}                 
 \def\Pb      {\ensuremath{\mathrm{b}}\xspace}                 
 \def\Pc      {\ensuremath{\mathrm{c}}\xspace}                 
 \def\Pd      {\ensuremath{\mathrm{d}}\xspace}                 
 \def\Pe      {\ensuremath{\mathrm{e}}\xspace}                 
 \def\Pf      {\ensuremath{\mathrm{f}}\xspace}                 
 \def\Pg      {\ensuremath{\mathrm{g}}\xspace}                 
 \def\Ph      {\ensuremath{\mathrm{h}}\xspace}                 
 \def\Pi      {\ensuremath{\mathrm{i}}\xspace}                 
 \def\Pj      {\ensuremath{\mathrm{j}}\xspace}                 
 \def\Pk      {\ensuremath{\mathrm{k}}\xspace}                 
 \def\Pl      {\ensuremath{\mathrm{l}}\xspace}                 
 \def\Pm      {\ensuremath{\mathrm{m}}\xspace}                 
 \def\Pn      {\ensuremath{\mathrm{n}}\xspace}                 
 \def\Po      {\ensuremath{\mathrm{o}}\xspace}                 
 \def\Pp      {\ensuremath{\mathrm{p}}\xspace}                 
 \def\Pq      {\ensuremath{\mathrm{q}}\xspace}                 
 \def\Pr      {\ensuremath{\mathrm{r}}\xspace}                 
 \def\Ps      {\ensuremath{\mathrm{s}}\xspace}                 
 \def\Pt      {\ensuremath{\mathrm{t}}\xspace}                 
 \def\Pu      {\ensuremath{\mathrm{u}}\xspace}                 
 \def\Pv      {\ensuremath{\mathrm{v}}\xspace}                 
 \def\Pw      {\ensuremath{\mathrm{w}}\xspace}                 
 \def\Px      {\ensuremath{\mathrm{x}}\xspace}                 
 \def\Py      {\ensuremath{\mathrm{y}}\xspace}                 
 \def\Pz      {\ensuremath{\mathrm{z}}\xspace}                 
}
{\def\Palpha      {\ensuremath{\alpha}\xspace}
 \def\Pbeta       {\ensuremath{\beta}\xspace}
 \def\Pgamma      {\ensuremath{\gamma}\xspace}                 
 \def\Pdelta      {\ensuremath{\delta}\xspace}                 
 \def\Pepsilon    {\ensuremath{\epsilon}\xspace}                 
 \def\Pvarepsilon {\ensuremath{\varepsilon}\xspace}                 
 \def\Pzeta       {\ensuremath{\zeta}\xspace}                 
 \def\Peta        {\ensuremath{\eta}\xspace}                 
 \def\Ptheta      {\ensuremath{\theta}\xspace}                 
 \def\Pvartheta   {\ensuremath{\vartheta}\xspace}                 
 \def\Piota       {\ensuremath{\iota}\xspace}                 
 \def\Pkappa      {\ensuremath{\kappa}\xspace}                 
 \def\Plambda     {\ensuremath{\lambda}\xspace}                 
 \def\Pmu         {\ensuremath{\mu}\xspace}                 
 \def\Pnu         {\ensuremath{\nu}\xspace}                 
 \def\Pxi         {\ensuremath{\xi}\xspace}                 
 \def\Ppi         {\ensuremath{\pi}\xspace}                 
 \def\Pvarpi      {\ensuremath{\varpi}\xspace}                 
 \def\Prho        {\ensuremath{\rho}\xspace}                 
 \def\Pvarrho     {\ensuremath{\varrho}\xspace}                 
 \def\Ptau        {\ensuremath{\tau}\xspace}                 
 \def\Pupsilon    {\ensuremath{\upsilon}\xspace}                 
 \def\Pphi        {\ensuremath{\phi}\xspace}                 
 \def\Pvarphi     {\ensuremath{\varphi}\xspace}                 
 \def\Pchi        {\ensuremath{\chi}\xspace}                 
 \def\Ppsi        {\ensuremath{\psi}\xspace}                 
 \def\Pomega      {\ensuremath{\omega}\xspace}                 
 \mathchardef\PDelta="7101
 \mathchardef\PXi="7104
 \mathchardef\PLambda="7103
 \mathchardef\PSigma="7106
 \mathchardef\POmega="710A
 \mathchardef\PUpsilon="7107
 \def\PA      {\ensuremath{A}\xspace}                 
 \def\PB      {\ensuremath{B}\xspace}                 
 \def\PC      {\ensuremath{C}\xspace}                 
 \def\PD      {\ensuremath{D}\xspace}                 
 \def\PE      {\ensuremath{E}\xspace}                 
 \def\PF      {\ensuremath{F}\xspace}                 
 \def\PG      {\ensuremath{G}\xspace}                 
 \def\PH      {\ensuremath{H}\xspace}                 
 \def\PI      {\ensuremath{I}\xspace}                 
 \def\PJ      {\ensuremath{J}\xspace}                 
 \def\PK      {\ensuremath{K}\xspace}                 
 \def\PL      {\ensuremath{L}\xspace}                 
 \def\PM      {\ensuremath{M}\xspace}                 
 \def\PN      {\ensuremath{N}\xspace}                 
 \def\PO      {\ensuremath{O}\xspace}                 
 \def\PP      {\ensuremath{P}\xspace}                 
 \def\PQ      {\ensuremath{Q}\xspace}                 
 \def\PR      {\ensuremath{R}\xspace}                 
 \def\PS      {\ensuremath{S}\xspace}                 
 \def\PT      {\ensuremath{T}\xspace}                 
 \def\PU      {\ensuremath{U}\xspace}                 
 \def\PV      {\ensuremath{V}\xspace}                 
 \def\PW      {\ensuremath{W}\xspace}                 
 \def\PX      {\ensuremath{X}\xspace}                 
 \def\PY      {\ensuremath{Y}\xspace}                 
 \def\PZ      {\ensuremath{Z}\xspace}                 
 \def\Pa      {\ensuremath{a}\xspace}                 
 \def\Pb      {\ensuremath{b}\xspace}                 
 \def\Pc      {\ensuremath{c}\xspace}                 
 \def\Pd      {\ensuremath{d}\xspace}                 
 \def\Pe      {\ensuremath{e}\xspace}                 
 \def\Pf      {\ensuremath{f}\xspace}                 
 \def\Pg      {\ensuremath{g}\xspace}                 
 \def\Ph      {\ensuremath{h}\xspace}                 
 \def\Pi      {\ensuremath{i}\xspace}                 
 \def\Pj      {\ensuremath{j}\xspace}                 
 \def\Pk      {\ensuremath{k}\xspace}                 
 \def\Pl      {\ensuremath{l}\xspace}                 
 \def\Pm      {\ensuremath{m}\xspace}                 
 \def\Pn      {\ensuremath{n}\xspace}                 
 \def\Po      {\ensuremath{o}\xspace}                 
 \def\Pp      {\ensuremath{p}\xspace}                 
 \def\Pq      {\ensuremath{q}\xspace}                 
 \def\Pr      {\ensuremath{r}\xspace}                 
 \def\Ps      {\ensuremath{s}\xspace}                 
 \def\Pt      {\ensuremath{t}\xspace}                 
 \def\Pu      {\ensuremath{u}\xspace}                 
 \def\Pv      {\ensuremath{v}\xspace}                 
 \def\Pw      {\ensuremath{w}\xspace}                 
 \def\Px      {\ensuremath{x}\xspace}                 
 \def\Py      {\ensuremath{y}\xspace}                 
 \def\Pz      {\ensuremath{z}\xspace}                 
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Leptons
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{\Pe}\xspace}
\def\en         {\ensuremath{\Pe^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{\Pe^+}\xspace}
\def\epm        {\ensuremath{\Pe^\pm}\xspace} 
\def\epem       {\ensuremath{\Pe^+\Pe^-}\xspace}
\def\ee         {\ensuremath{\Pe^-\Pe^-}\xspace}

\def\mmu        {\ensuremath{\Pmu}\xspace}
\def\mup        {\ensuremath{\Pmu^+}\xspace}
\def\mun        {\ensuremath{\Pmu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\Pmu^+\Pmu^-}\xspace}
\def\mtau       {\ensuremath{\Ptau}\xspace}

\def\taup       {\ensuremath{\Ptau^+}\xspace}
\def\taum       {\ensuremath{\Ptau^-}\xspace}
\def\tautau     {\ensuremath{\Ptau^+\Ptau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\neu        {\ensuremath{\Pnu}\xspace}
\def\neub        {\ensuremath{\overline{\Pnu}}\xspace}
\def\nuenueb      {\ensuremath{\neu\neub}\xspace}
\def\neue        {\ensuremath{\neu_e}\xspace}
\def\neueb       {\ensuremath{\neub_e}\xspace}
\def\neueneueb    {\ensuremath{\neue\neueb}\xspace}
\def\neum        {\ensuremath{\neu_\mu}\xspace}
\def\neumb       {\ensuremath{\neub_\mu}\xspace}
\def\neumneumb    {\ensuremath{\neum\neumb}\xspace}
\def\neut        {\ensuremath{\neu_\tau}\xspace}
\def\neutb       {\ensuremath{\neub_\tau}\xspace}
\def\neutneutb    {\ensuremath{\neut\neutb}\xspace}
\def\neul        {\ensuremath{\neu_\ell}\xspace}
\def\neulb       {\ensuremath{\neub_\ell}\xspace}
\def\neulneulb    {\ensuremath{\neul\neulb}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Gauge bosons and scalars
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g      {\ensuremath{\Pgamma}\xspace}
\def\H      {\ensuremath{\PH^0}\xspace}
\def\Hp     {\ensuremath{\PH^+}\xspace}
\def\Hm     {\ensuremath{\PH^-}\xspace}
\def\Hpm    {\ensuremath{\PH^\pm}\xspace}
\def\W      {\ensuremath{\PW}\xspace}
\def\Wp     {\ensuremath{\PW^+}\xspace}
\def\Wm     {\ensuremath{\PW^-}\xspace}
\def\Wpm    {\ensuremath{\PW^\pm}\xspace}
\def\Z      {\ensuremath{\PZ^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Quarks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{\Pq}\xspace}
\def\qbar  {\ensuremath{\overline \q}\xspace}
\def\qqbar {\ensuremath{\q\qbar}\xspace}
\def\u     {\ensuremath{\Pu}\xspace}
\def\ubar  {\ensuremath{\overline \u}\xspace}
\def\uubar {\ensuremath{\u\ubar}\xspace}
\def\d     {\ensuremath{\Pd}\xspace}
\def\dbar  {\ensuremath{\overline \d}\xspace}
\def\ddbar {\ensuremath{\d\dbar}\xspace}
\def\s     {\ensuremath{\Ps}\xspace}
\def\sbar  {\ensuremath{\overline \s}\xspace}
\def\ssbar {\ensuremath{\s\sbar}\xspace}
\def\c     {\ensuremath{\Pc}\xspace}
\def\cbar  {\ensuremath{\overline \c}\xspace}
\def\ccbar {\ensuremath{\c\cbar}\xspace}
\def\b     {\ensuremath{\Pb}\xspace}
\def\bbar  {\ensuremath{\overline \b}\xspace}
\def\bbbar {\ensuremath{\b\bbar}\xspace}
\def\t     {\ensuremath{\Pt}\xspace}
\def\tbar  {\ensuremath{\overline \t}\xspace}
\def\ttbar {\ensuremath{\t\tbar}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Light mesons
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\pion  {\ensuremath{\Ppi}\xspace}
\def\piz   {\ensuremath{\pion^0}\xspace}
\def\pizs  {\ensuremath{\pion^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pion^0\pion^0}\xspace}
\def\pip   {\ensuremath{\pion^+}\xspace}
\def\pim   {\ensuremath{\pion^-}\xspace}
\def\pipi  {\ensuremath{\pion^+\pion^-}\xspace}
\def\pipm  {\ensuremath{\pion^\pm}\xspace}
\def\pimp  {\ensuremath{\pion^\mp}\xspace}

\def\kaon  {\ensuremath{\PK}\xspace}
%%% do NOT use ensuremath here
  \def\Kbar  {\kern 0.2em\overline{\kern -0.2em \PK}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{\kaon^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{\kaon^+}\xspace}
\def\Km    {\ensuremath{\kaon^-}\xspace}
\def\Kpm   {\ensuremath{\kaon^\pm}\xspace}
\def\Kmp   {\ensuremath{\kaon^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{\kaon^0_{\rm\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{\kaon^0_{\rm\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{\kaon^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{\kaon^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{\kaon^{*+}}\xspace}
\def\Kstarm  {\ensuremath{\kaon^{*-}}\xspace}
\def\Kstarpm {\ensuremath{\kaon^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{\kaon^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\Peta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Heavy mesons
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
  \def\Dbar    {\kern 0.2em\overline{\kern -0.2em \PD}{}\xspace}
\def\D       {\ensuremath{\PD}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{\D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{\D^+}\xspace}
\def\Dm      {\ensuremath{\D^-}\xspace}
\def\Dpm     {\ensuremath{\D^\pm}\xspace}
\def\Dmp     {\ensuremath{\D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{\D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{\D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{\D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{\D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{\D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{\D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{\D^+_s}\xspace}
\def\Dsminus      {\ensuremath{\D^-_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{\D^{*+}_s}\xspace}
\def\Dspm    {\ensuremath{\D^{\pm}_s}\xspace}


\def\B       {\ensuremath{\PB}\xspace}
%%% do NOT use ensuremath here
  \def\Bbar    {\kern 0.18em\overline{\kern -0.18em \PB}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BBbar   {\ensuremath{\B\Bbar}\xspace} 
\def\Bz      {\ensuremath{\B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\Bu      {\ensuremath{\B^+}\xspace}
\def\Bub     {\ensuremath{\B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{\B^\pm}\xspace}
\def\Bmp     {\ensuremath{\B^\mp}\xspace}
\def\Bd      {\ensuremath{\B^0}\xspace}
\def\Bs      {\ensuremath{\B^0_s}\xspace}
\def\Bq      {\ensuremath{\B_q}\xspace}
\def\Bqbar      {\ensuremath{\bar{\B_q}}\xspace}
\def\Bsb     {\ensuremath{\Bbar^0_s}\xspace}
\def\Bsbar     {\ensuremath{\Bbar^0_s}\xspace}
\def\Bdb     {\ensuremath{\Bbar^0}\xspace}
\def\Bdbar     {\ensuremath{\Bbar^0}\xspace}
\def\Bc      {\ensuremath{\B_c^+}\xspace}
\def\Bcb     {\ensuremath{\B_c^-}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Onia
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}\xspace}
%\def\Jpsi     {\ensuremath{{\PJ\mskip -3mu/\mskip -2mu\Ppsi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\Ppsi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\Ppsi(3770)}\xspace}
\def\etac     {\ensuremath{\Peta_c}\xspace}
\def\chiczero {\ensuremath{\Pchi_{c0}}\xspace}
\def\chicone  {\ensuremath{\Pchi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\Pchi_{c2}}\xspace}
  %\mathchardef\Upsilon="7107
  \def\Y#1S{\ensuremath{\PUpsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

\def\chic  {\ensuremath{\Pchi_{c}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Baryons
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{\Pp}\xspace}
\def\antiproton  {\ensuremath{\overline \proton}\xspace}
\def\neutron     {\ensuremath{\Pn}\xspace}
\def\antineutron {\ensuremath{\overline \neutron}\xspace}

\def\Deltares {\ensuremath{\PDelta}\xspace}
\def\Deltaresbar{\ensuremath{\overline \Deltares}\xspace}
\def\Xires {\ensuremath{\PXi}\xspace}
\def\Xiresbar{\ensuremath{\overline \Xires}\xspace}
\def\L {\ensuremath{\PLambda}\xspace}
\def\Lbar{\ensuremath{\overline \L}\xspace}
\def\Lambdares {\ensuremath{\PLambda}\xspace}
\def\Lambdaresbar{\ensuremath{\overline \Lambdares}\xspace}
\def\Sigmares {\ensuremath{\PSigma}\xspace}
\def\Sigmaresbar{\ensuremath{\overline \Sigmares}\xspace}
\def\Omegares {\ensuremath{\POmega}\xspace}
\def\Omegaresbar{\ensuremath{\overline \Omegares}\xspace}

%%% do NOT use ensuremath here
 % \def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
 % \def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
 % \def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
 % \def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
 % \def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
 % \def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
 % \def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\Lb      {\ensuremath{\L_b}\xspace}
\def\Lbbar   {\ensuremath{\Lbar_b}\xspace}
\def\Lc      {\ensuremath{\L_c}\xspace}
\def\Lcbar   {\ensuremath{\Lbar_c}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Lifetimes
\newcommand{\tauBs}{\ensuremath{\tau_{\Bs}}\xspace}
\newcommand{\tauBd}{\ensuremath{\tau_{\B}}\xspace}
\newcommand{\tauBz}{\ensuremath{\tau_{\B}}\xspace}
\newcommand{\tauBu}{\ensuremath{\tau_{\Bp}}\xspace}
\newcommand{\tauDp}{\ensuremath{\tau_{\Dp}}\xspace}
\newcommand{\tauDz}{\ensuremath{\tau_{\Dz}}\xspace}
\newcommand{\tauL}{\ensuremath{\tau_{\rm L}}\xspace}
\newcommand{\tauH}{\ensuremath{\tau_{\rm H}}\xspace}

%% Masses
\newcommand{\mBd}{\ensuremath{m_{\Bd}}\xspace}
\newcommand{\mBp}{\ensuremath{m_{\Bp}}\xspace}
\newcommand{\mBs}{\ensuremath{m_{\Bs}}\xspace}
\newcommand{\mBc}{\ensuremath{m_{\Bc}}\xspace}
\newcommand{\mLb}{\ensuremath{m_{\Lb}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Units
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\unit}[1]{\ensuremath{\rm\,#1}\xspace}          % {kg}

%% Energy and momentum
\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\TeV}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\gevgevcccc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V^2\!/}c^4}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}

%% Distance and area
\def\km   {\ensuremath{\rm \,km}\xspace}
\def\m    {\ensuremath{\rm \,m}\xspace}
\def\cm   {\ensuremath{\rm \,cm}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{\rm \,mm}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
\def\mum  {\ensuremath{\,\upmu\rm m}\xspace}
\def\muma {\ensuremath{\,\upmu\rm m^2}\xspace}
\def\nm   {\ensuremath{\rm \,nm}\xspace}
\def\fm   {\ensuremath{\rm \,fm}\xspace}
\def\nm   {\ensuremath{\rm \,nm}\xspace}
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mub{\ensuremath{\rm \,\upmu b}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}
\def\invpb   {\ensuremath{\mbox{\,pb}^{-1}}\xspace}

%% Time and mass
\def\sec  {\ensuremath{\rm {\,s}}\xspace}
\def\ms   {\ensuremath{{\rm \,ms}}\xspace}
\def\mus  {\ensuremath{\,\upmu{\rm s}}\xspace}
\def\ns   {\ensuremath{{\rm \,ns}}\xspace}
\def\ps   {\ensuremath{{\rm \,ps}}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}

\def\mhz  {\ensuremath{{\rm \,MHz}}\xspace}
\def\khz  {\ensuremath{{\rm \,kHz}}\xspace}
\def\hz   {\ensuremath{{\rm \,Hz}}\xspace}

\def\invps{\ensuremath{{\rm \,ps^{-1}}}\xspace}


%% Decays
\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRvis      {{\ensuremath{\BR_{\rm{vis}}}}}
\newcommand{\decay}[2]{\ensuremath{#1\!\to #2}\xspace}         % {\Pa}{\Pb \Pc}
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Kinematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\et         {\mbox{$E_T$}\xspace}

%% Geometry
\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}

% QCD parameters
\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

% CKM, CP violation

\def\eps   {\ensuremath{\varepsilon}\xspace}
\def\epsK  {\ensuremath{\varepsilon_K}\xspace}
\def\epsB  {\ensuremath{\varepsilon_B}\xspace}
\def\epsp  {\ensuremath{\varepsilon^\prime_K}\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}

\def\Vud  {\ensuremath{V_{ud}}\xspace}
\def\Vcd  {\ensuremath{V_{cd}}\xspace}
\def\Vtd  {\ensuremath{V_{td}}\xspace}
\def\Vus  {\ensuremath{V_{us}}\xspace}
\def\Vcs  {\ensuremath{V_{cs}}\xspace}
\def\Vts  {\ensuremath{V_{ts}}\xspace}
\def\Vub  {\ensuremath{V_{ub}}\xspace}
\def\Vcb  {\ensuremath{V_{cb}}\xspace}
\def\Vtb  {\ensuremath{V_{tb}}\xspace}

% QM
\newcommand{\bra}[1]{\ensuremath{\langle #1|}}             % {a}
\newcommand{\ket}[1]{\ensuremath{|#1\rangle}}              % {b}
\newcommand{\braket}[2]{\ensuremath{\langle #1|#2\rangle}} % {a}{b}

%%  Miscellaneous
\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}

\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}
\def\rad{\ensuremath{\rm \,rad}\xspace}

\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

\def\order{{\ensuremath{\cal O}}\xspace}



\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{L}}\xspace}

\def\deriv {\ensuremath{\mathrm{d}}}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Programs
\def\evtgen     {\mbox{\textsc{EvtGen}}\xspace}
\def\pythia     {\mbox{\textsc{Pythia}}\xspace}
\def\fluka      {\mbox{\textsc{Fluka}}\xspace}
\def\geant      {\mbox{\textsc{GEANT}}\xspace}
\def\root       {\mbox{\textsc{ROOT}}\xspace}
\def\hepmc      {\mbox{\textsc{HepMC}}\xspace}
\def\gauss      {\mbox{\textsc{Gauss}}\xspace}
\def\gaudi      {\mbox{\textsc{Gaudi}}\xspace}
\def\brunel     {\mbox{\textsc{Brunel}}\xspace}
\def\davinci    {\mbox{\textsc{DaVinci}}\xspace}
\def\ganga      {\mbox{\textsc{Ganga}}\xspace}
\def\dirac      {\mbox{\textsc{DIRAC}}\xspace}
\def\root       {\mbox{\textsc{Root}}\xspace}
\def\roofit     {\mbox{\textsc{RooFit}}\xspace}
\def\pyroot     {\mbox{\textsc{PyROOT}}\xspace}

%% Languages
\def\cpp        {\mbox{\textsc{C\raisebox{0.1em}{{\footnotesize{++}}}}\xspace}}
\def\python     {\mbox{\textsc{Python}}\xspace}
\def\ruby       {\mbox{\textsc{Ruby}}\xspace}
\def\fortran    {\mbox{\textsc{FORTRAN}}\xspace}


%% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Key channels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\BdToKstmm    {\decay{\Bd}{\Kstarz\mup\mun}\xspace}
\def\BdbToKstmm   {\decay{\Bdb}{\Kstarzb\mup\mun}\xspace}

\def\BsToJPsiKK  {\decay{\Bs}{\jpsi\Kp\Km}\xspace}   
\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}\xspace}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}\xspace}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}\xspace}
\def\BdToJPsiKS   {\decay{\Bd}{\jpsi\KS}\xspace}

\def\BsPhiGam     {\decay{\Bd}{\phi \g}\xspace}
\def\BdKstGam     {\decay{\Bd}{\Kstarz \g}\xspace}

\def\BTohh        {\decay{\B}{\Ph^+ \Ph^-}\xspace}
\def\BdTopipi     {\decay{\Bd}{\pip\pim}\xspace}
\def\BdToKpi      {\decay{\Bd}{\Kp\pim}\xspace}
\def\BsToKK       {\decay{\Bs}{\Kp\Km}\xspace}
\def\BsDspi       {\decay{\Bs}{\Dsminus\pi^+}\xspace}
\def\BsDsmu       {\decay{\Bs}{\Dsminus\mu^+ \nu_\mu}\xspace}
\def\BsTopiK      {\decay{\Bs}{\pip\Km}\xspace}


\def\BdJmmKpi    {\decay{\Bd}{\jpsi(\mup\mun)\Kstarz(K\pi)}\xspace}
%\def\BdJKst      {\decay{\Bd}{\jpsi\Kstarz}\xspace}
%\def\BuJK        {\decay{\Bu}{\jpsi K^+}\xspace}
%\def\BdJKS       {\decay{\Bd}{\jpsi \KS}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Rare Decays
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Kinematics
\def\qsq       {\ensuremath{q^2}\xspace}
\def\ctl       {\ensuremath{\cos{\theta_l}}\xspace}
\def\ctk       {\ensuremath{\cos{\theta_K}}\xspace}

%% Decays
\def\BdKstee  {\decay{\Bd}{\Kstarz\epem}\xspace}
\def\BdbKstee {\decay{\Bdb}{\Kstarzb\epem}\xspace}
\def\bsll     {\decay{\b}{\s \ell^+ \ell^-}\xspace}
\def\AFB      {\ensuremath{A_{\mathrm{FB}}}\xspace}
\def\AT#1     {\ensuremath{A_T^{#1}}\xspace}           % 2
\def\btosgam  {\decay{\b}{\s \g}\xspace}
\def\btodgam  {\decay{\b}{\d \g}\xspace}
\def\Bsmm     {\decay{\Bs}{\mup\mun}\xspace}
\def\Bdmm     {\decay{\Bd}{\mup\mun}\xspace}

%% Wilson coefficients and operators
\def\C#1      {\ensuremath{\mathcal{C}_{#1}}}                       % 9
\def\Cp#1     {\ensuremath{\mathcal{C}_{#1}^{'}}}                    % 7
\def\Ceff#1   {\ensuremath{\mathcal{C}_{#1}^{\mathrm{(eff)}}}}        % 9  
\def\Cpeff#1  {\ensuremath{\mathcal{C}_{#1}^{'\mathrm{(eff)}}}}       % 7
\def\Ope#1    {\ensuremath{\mathcal{O}_{#1}}}                       % 2
\def\Opep#1   {\ensuremath{\mathcal{O}_{#1}^{'}}}                    % 7

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% B oscillations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Decays
\newcommand{\dm}{\ensuremath{\Delta m}}
\newcommand{\dms}{\ensuremath{\Delta m_{\s}}}
\newcommand{\dmd}{\ensuremath{\Delta m_{\d}}}
\newcommand{\DG}{\ensuremath{\Delta\Gamma}}
\newcommand{\DGs}{\ensuremath{\Delta\Gamma_{\s}}}
\newcommand{\DGd}{\ensuremath{\Delta\Gamma_{\d}}}
\newcommand{\Gs}{\ensuremath{\Gamma_{\s}}}
\newcommand{\Gd}{\ensuremath{\Gamma_{\d}}}

\newcommand{\MBq}{\ensuremath{M_{\B_\q}}}
\newcommand{\DGq}{\ensuremath{\Delta\Gamma_{\q}}}
\newcommand{\Gq}{\ensuremath{\Gamma_{\q}}}
\newcommand{\dmq}{\ensuremath{\Delta m_{\q}}}
\newcommand{\GL}{\ensuremath{\Gamma_{\rm L}}}
\newcommand{\GH}{\ensuremath{\Gamma_{\rm H}}}

\newcommand{\DGsGs}{\ensuremath{\Delta\Gamma_{\s}/\Gamma_{\s}}}
\newcommand{\Delm}{\mbox{$\Delta m $}}
\newcommand{\ACP}{\ensuremath{{\cal A}^{\rm CP}}}
\newcommand{\Adir}{\ensuremath{{\cal A}^{\rm dir}}}
\newcommand{\Amix}{\ensuremath{{\cal A}^{\rm mix}}}
\newcommand{\ADelta}{\ensuremath{{\cal A}^\Delta}}
%\newcommand{\phid}{\ensuremath{\phi_{\d}}}
\newcommand{\sinphid}{\ensuremath{\sin\!\phid}}
\newcommand{\phis}{\ensuremath{\phi_{\s}}}
\newcommand{\betas}{\ensuremath{\beta_{\s}}}
\newcommand{\sbetas}{\ensuremath{\sigma(\beta_{\s})}}
\newcommand{\stbetas}{\ensuremath{\sigma(2\beta_{\s})}}
\newcommand{\stphis}{\ensuremath{\sigma(\phi_{\s})}}
\newcommand{\sinphis}{\ensuremath{\sin\!\phis}}

%% Tagging
\newcommand{\edet}{{\ensuremath{\varepsilon_{\rm det}}}}
\newcommand{\erec}{{\ensuremath{\varepsilon_{\rm rec/det}}}}
\newcommand{\esel}{{\ensuremath{\varepsilon_{\rm sel/rec}}}}
\newcommand{\etrg}{{\ensuremath{\varepsilon_{\rm trg/sel}}}}
\newcommand{\etot}{{\ensuremath{\varepsilon_{\rm tot}}}}

\newcommand{\mistag}{\ensuremath{\omega}}
\newcommand{\wcomb}{\ensuremath{\omega^{\rm comb}}}
\newcommand{\etag}{{\ensuremath{\varepsilon_{\rm tag}}}}
\newcommand{\etagcomb}{{\ensuremath{\varepsilon_{\rm tag}^{\rm comb}}}}
\newcommand{\effeff}{\ensuremath{\varepsilon_{\rm eff}}}
\newcommand{\effeffcomb}{\ensuremath{\varepsilon_{\rm eff}^{\rm comb}}}
\newcommand{\efftag}{{\ensuremath{\etag(1-2\omega)^2}}}
\newcommand{\effD}{{\ensuremath{\etag D^2}}}
\newcommand{\etagprompt}{{\ensuremath{\varepsilon_{\rm tag}^{\rm Pr}}}}
\newcommand{\etagLL}{{\ensuremath{\varepsilon_{\rm tag}^{\rm LL}}}}

%% User
%\def\sim                 {\ensuremath{\sim}\xspace}
\def\BdToDstmunu  {\decay{\Bz}{\Dstarm \mup \neum}\xspace}
\def\BsToJPsiPhi  {\decay{\Bs}{\jpsi\phi}\xspace}
%\def\BsJphi  {\decay{\Bs}{\jpsi\phi}\xspace}
\def\BdToJPsiKst  {\decay{\Bd}{\jpsi\Kstarz}\xspace}
%\def\BdJKst  {\decay{\Bd}{\jpsi\Kstarz}\xspace}
\def\BdbToJPsiKst {\decay{\Bdb}{\jpsi\Kstarzb}\xspace}
\def\BuToJPsiKp {\decay{\Bu}{\jpsi\Kp}}
\def\BsToDspi {\decay{\Bs}{\Ds\pim}}
\def\BToJPsiX  {\decay{\B}{\jpsi X}\xspace}

\newcommand{\bs}{\BsToJPsiPhi}
\newcommand{\bplus}{\BuToJPsiKp}
\newcommand{\bkstar}{\BdToJPsiKst}
\newcommand{\dspi}{\BsToDspi}
\newcommand{\dstarmunu}{\BdToDstmunu}
\newcommand{\Dilu}{{\ensuremath{D}}} % Stefania
\newcommand{\chidof}{\ensuremath{\chi^2/d.o.f}~} 


% from roadmap:
%\newcommand{\phijphi}{\ensuremath{\phi_s^{\jpsi\phi}}}
\newcommand{\phijphi}{\ensuremath{\phi_s}}
\newcommand{\Jphi}{\ensuremath{\jpsi\phi}}
\def\thetatwo{\theta_2}
\def\apar{A_{\|}(t)}
\def\aperp{A_{\perp}(t)}
\def\azero{A_{0}(t)}
\def\aparO{A_{\|}(0)}
\def\aperpO{A_{\perp}(0)}
\def\azeroO{A_{0}(0)}
\newcommand{\Rt}{R_\perp}
\newcommand{\Rp}{R_\|}
\newcommand{\Ro}{R_0}
\newcommand{\dGtwo}{\frac{\DG}{2}}
\renewcommand{\d}{{\rm d}}

\def\aparb{\bar{A}_{\|}(t)}
\def\aperpb{\bar{A}_{\perp}(t)}
\def\azerob{\bar{A}_{0}(t)}
\def\aparbO{\bar{A}_{\|}(0)}
\def\aperpbO{\bar{A}_{\perp}(0)}
\def\azerobO{\bar{A}_{0}(0)}

\newcommand{\delone}{\delta_1}
\newcommand{\deltwo}{\delta_2}
%\newcommand{\delperp}{\delta_{\perp}}
%\newcommand{\delpar}{\delta_{\|}}
%\newcommand{\delzero}{\delta_0}

\newcommand{\thetatr}{\ensuremath{\theta}}
\newcommand{\phitr}{\ensuremath{\varphi}}
\newcommand{\psitr}{\ensuremath{\psi}}
\newcommand{\thetaone}{\ensuremath{\psi}}



\newcommand{\Bqq}{\ensuremath{B_q}}
\newcommand{\Bqqbar}{\ensuremath{\bar{B_q}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\calH}{\ensuremath{{\cal H}}}
\newcommand{\BL}{\ensuremath{B_L}}
\newcommand{\BH}{\ensuremath{B_H}}
\newcommand{\BLH}{\ensuremath{B_{L,H}}}

\newcommand{\Af}{\ensuremath{A_{f}}}
\newcommand{\Afbar}{\ensuremath{\overline{A}_{\overline{f}}}}
\newcommand{\fbar}{\ensuremath{\bar{ f}}}
\newcommand{\SM}{Standard Model}
\newcommand{\bccsbar}{\decay{\BAR{b}}{\BAR{c}c\BAR{s}}}


\newcommand{\phiM}{\ensuremath{\Phi_{\rm M}}}
\newcommand{\phiD}{\ensuremath{\Phi_{\rm D}}}
\newcommand{\phiCP}{\ensuremath{\Phi_{\rm CP}}}
\newcommand{\phiMNP}{\ensuremath{\Phi^{\rm NP}_{\rm M}}}
\newcommand{\phiDNP}{\ensuremath{\Phi^{\rm NP}_{\rm D}}}
\newcommand{\phiMG}{\ensuremath{\phi_{\rm s}^{\rm M/\Gamma}}}
\newcommand{\phiMGSM}{\ensuremath{\phi^{\rm M/\Gamma}_{\rm s \, ,SM}}}

\newcommand{\phipen}{\ensuremath{\Phi_{\rm penguin}}}
\newcommand{\phibox}{\ensuremath{\Phi_{\rm box}}}

\newcommand{\phiNP}{\ensuremath{\Phi^{\rm NP}}}
\newcommand{\phiSM}{\ensuremath{\phi_s^{\rm SM}}}
\newcommand{\phisDelta}{\ensuremath{\phi^\Delta_{\rm s}}}
\newcommand{\phitot}{\ensuremath{\Phi_{\rm tot}}}

\newcommand{\diffX}{ \frac{\d^{4} \Gamma}{\d t\, \d\Omega} }
\newcommand{\diffXbar}{ \frac{\d^{4} \bar \Gamma}{\d t\, \d\Omega} }

%\newcommand{\phiKK}{\ensuremath{\phi\to K^+K^-}}
\newcommand{\Kplus}{\ensuremath{K^+}}
\newcommand{\bb}{\ensuremath{b\bar{b}}}
%\newcommand{\pT}{\ensuremath{p_{\rm T}}}

% New commands from roadmap
\newcommand{\particle}[1]{{\ensuremath{\rm #1}}}
%\newcommand{\Jpsi}{\particle{J\!/\!\psi}}
\newcommand{\Jpsi}{\ensuremath{J\!/\!\psi}}
\newcommand{\Jmm}{\particle{\Jpsi(\mu\mu)}}
\newcommand{\Jee}{\particle{\Jpsi(ee)}}
\newcommand{\JpsiX}{\particle{\Jpsi X}}
%\newcommand{\DLL}[2]{\ensuremath{\Delta  \ln{\cal L}_{\particle{#1}\particle{#2}}}}
\newcommand{\BuJK}{\decay{\Bu}{\Jpsi K^+}}               %         Bu->JpsiK  
%\newcommand{\Kplus}{\particle{K^+}}
\newcommand{\Kminus}{\particle{K^-}}
%\newcommand{\Kst}{\particle{K^{*0}}}
\newcommand{\Kst}{\ensuremath{K^{*0}}}
\newcommand{\Kstbar}{\particle{\BAR{K}^{*0}}}
\newcommand{\Kpi}{\particle{K^+\pi^-}}
\newcommand{\BsJphi}{\decay{\Bs}{\Jpsi\phi}}             %         Bs->Jpsiphi  
\newcommand{\BsJmmphiKK}{\decay{\Bs}{\Jpsi(\mu^+\mu^-)\phi(K^+K^-)}}             %         Bs->Jpsiphi  
\newcommand{\BdJKst}{\decay{\Bd}{\Jpsi\Kst}}             %         Bd->JpsiK*  
\newcommand{\BdJKS}{\decay{\Bd}{\Jpsi\KS}}               %         Bd->JpsiKS  
\newcommand{\KstKpi}{\decay{\Kst}{\Kpi}}
\newcommand{\phiKK}{\decay{\phi}{K^+K^-}}
\newcommand{\pT}{\ensuremath{p_{\rm T}}}
\newcommand{\pTmin}{\ensuremath{\pT^{\rm min}}}
\newcommand{\GeVc}{\unit{GeV\!/\!{\it c}}}
\newcommand{\MeVc}{\unit{MeV\!/\!{\it c}}}
\newcommand{\MeVcc}{\unit{MeV\!/\!{\it c}^2}}
\newcommand{\GeVcc}{\unit{MeV\!/\!{\it c}^2}}
\newcommand{\GeV}{\unit{GeV}}

\newcommand{\Jpsimm}{\decay{\Jpsi}{\mu\mu}}
\newcommand{\BdJmmKst}{\decay{\Bd}{\Jmm\Kst(\particle{K}\pi)}}            %  411500 Bd->Jpsi(mumu)K*  
\newcommand{\BuJmmK}{\decay{\Bu}{\Jmm K^+}}              %         Bu->Jpsi(mumu)K  
\newcommand{\BsJmmphi}{\decay{\Bs}{\Jmm\phi(\particle{KK})}}            %  611300 Bs->Jpsi(mumu)phi  
\newcommand{\BJX}{\decay{B}{\Jpsi X}}
\newcommand{\KSpipi}{\decay{K^0_S}{\pi^+\pi^-}}
\newcommand{\Lppi}{\decay{\Lambda}{p^+\pi^-}}
\newcommand{\LbJL}{\decay{\Lambda_b}{\Jpsi\Lambda}}             %         Bs->Jpsiphi  
\newcommand{\BdJmmKS}{\decay{\Bd}{\Jmm\KS(\pi\pi)}}              %  411300 Bd->Jpsi(mumu)KS  
\newcommand{\LbJmmL}{\decay{\Lambda_b}{\Jmm\Lambda(p\pi)}}              %  411300 Bd->Jpsi(mumu)KS  


% from note2:
%\newcommand{\bdjpsimmkstar}{\ensuremath{\textrm{B}_{\textrm{d}}\rightarrow
%                      J/\psi(\mu^{+} \mu^{-}) K^{*}}}
%\newcommand{\bsjpsimmphi}{\ensuremath{\textrm{B}_{\textrm{s}}\rightarrow
%                      J/\psi(\mu^{+} \mu^{-}) \phi(K^{+} K^{-})}}
\def\etal{{\em et al}}
%%a lot of these are already defined int he symbol list
%\newcommand{\dg}{\ensuremath{\Delta\Gamma}}
%\newcommand{\gs}{\ensuremath{\Gamma_s}}
%\newcommand{\gl}{\ensuremath{\Gamma_L}}
%\newcommand{\gh}{\ensuremath{\Gamma_H}}
%%\newcommand{\dspi}{\ensuremath{\textrm{B}_\textrm{s}\rightarrow D_s\pi}}
%\newcommand{\dsds}{\ensuremath{\textrm{B}_\textrm{s}\rightarrow \textrm{D}_\textrm{s} \textrm{D}_\textrm{s}}}
%\newcommand{\dsmunu}{\ensuremath{\textrm{B}_\textrm{s}\rightarrow D_\textrm{s}\mu\nu}}
%\newcommand{\jpsiphi}{\ensuremath{\textrm{B}_\textrm{s}^0\rightarrow J/\psi\phi}}
%\newcommand{\jpsiKstar}{\ensuremath{\textrm{B}_\textrm{d}^0\rightarrow J/\psi \textrm{K}^*}}
%\newcommand{\jpsiK}{\ensuremath{\textrm{B}_\textrm{u}\rightarrow \textrm{J}/\psi \textrm{K}}}
%\newcommand{\inclusive}{\ensuremath{\textrm{B}\rightarrow \textrm{J}/\psi \textrm{X}}}
%\newcommand{\bs}{\ensuremath{\textrm{B}_\textrm{s}^0}}
%\newcommand{\bd}{\ensuremath{\textrm{B}_\textrm{d}^0}}


% Uli
\newcommand{\magsq}[1]{\ensuremath{\left| #1 \right|^2}}
\newcommand{\modulus}[1]{\ensuremath{\left| #1 \right|}}
\newcommand{\of}[1]{\ensuremath{\left( #1 \right)}}
\newcommand{\brackets}[1]{\ensuremath{\left[ #1 \right]}}

\newcommand{\gd}{\ensuremath{\Gamma_d}}
\newcommand{\dgs}{\ensuremath{\Delta\Gamma_s}}
\newcommand{\bsb}{\ensuremath{\bar{\textrm{B}}_\textrm{s}}}
\newcommand{\bdb}{\ensuremath{\bar{\textrm{B}}_\textrm{d}}}
\newcommand{\bq}{\ensuremath{\textrm{B}_\textrm{q}^0}}
\newcommand{\bqb}{\ensuremath{\bar{\textrm{B}}_\textrm{q}^0}}
\newcommand{\bqbar}{\ensuremath{\bar{\textrm{B}}_\textrm{q}^0}}
\newcommand{\bqh}{\ensuremath{\textrm{B}_{\textrm{q}H}}}
\newcommand{\bql}{\ensuremath{\textrm{B}_{\textrm{q}L}}}
% \newcommand{\dm}{\ensuremath{\Delta m}}
\newcommand{\gql}{\ensuremath{\Gamma_{\textrm{q}L}}}
\newcommand{\gqh}{\ensuremath{\Gamma_{\textrm{q}H}}}
\newcommand{\dgq}{\ensuremath{\Delta\Gamma_q}}
\newcommand{\gq}{\ensuremath{\Gamma_q}}
% end Uli

%amplitudes and phases
%\newcommand{\delone}{\delta_1}
%\newcommand{\deltwo}{\delta_2}
\newcommand{\delperp}{\ensuremath{\delta_{\perp}}}
\newcommand{\delpar}{\ensuremath{\delta_{\|}}}
\newcommand{\delzero}{\ensuremath{\delta_0}}
%\def\thetatwo{\theta_2}
%\def\apar{A_{\|}(t)}
%\def\aperp{A_{\perp}(t)}
%\def\azero{A_{0}(t)}
%\def\aparO{A_{\|}(0)}
%\def\aperpO{A_{\perp}(0)}
%\def\azeroO{A_{0}(0)}
%\newcommand{\Rt}{R_\perp}
%\newcommand{\Rp}{R_\|}
%\newcommand{\Ro}{R_0}
%\newcommand{\dGtwo}{\frac{\DG}{2}}
%\renewcommand{\d}{{\rm d}}
%\def\aparb{\bar{A}_{\|}(t)}
%\def\aperpb{\bar{A}_{\perp}(t)}
%\def\azerob{\bar{A}_{0}(t)}
%\def\aparbO{\bar{A}_{\|}(0)}
%\def\aperpbO{\bar{A}_{\perp}(0)}
%\def\azerobO{\bar{A}_{0}(0)}

%\newcommand{\thetatr}{\ensuremath{\theta}}
%\newcommand{\phitr}{\ensuremath{\varphi}}
%\newcommand{\psitr}{\ensuremath{\psi}}
%\newcommand{\thetaone}{\ensuremath{\psi}}

\newcommand{\fsig}{\ensuremath{f_\text{sig}}}
\newcommand{\fbkg}{\ensuremath{f_\text{bkg}^1}}
\newcommand{\sigmam}{\ensuremath{\sigma_{m}}}
\newcommand{\alpham}{\ensuremath{\alpha_{m}}}
\newcommand{\taubkgO}{\ensuremath{\tau_\text{bkg,1}}}
\newcommand{\taubkgI}{\ensuremath{\tau_\text{bkg,2}}}
\newcommand{\lambdaphys}{\ensuremath{\lambda_\text{phys}}}
\newcommand{\lambdadet}{\ensuremath{\lambda_\text{det}}}
\newcommand{\lambdabkg}{\ensuremath{\lambda_\text{bkg}}}
\newcommand{\fsigmat}{\ensuremath{f_\sigma^t}}
\newcommand{\sigmatO}{\ensuremath{\sigma_{t,1}}}
\newcommand{\sigmatI}{\ensuremath{\sigma_{t,2}}}
%
%
%
\newcommand{\dtheta}{\ensuremath{\text{dcos}\thetatr}}
\newcommand{\dpsi}{\ensuremath{\text{dcos}\psitr}}
\newcommand{\dphi}{\ensuremath{\text{d}\phitr}}
\newcommand{\dt}{\ensuremath{\text{dt}}}

\newcommand{\abssq}[1]{\ensuremath{\lvert #1 \rvert^2}}
\newcommand{\abs}[1]{\ensuremath{\lvert #1 \rvert}}

\newcommand{\comment}[1]{\par\noindent {\em\small [#1]}}
\renewcommand{\comment}[1]{}

%\newcommand\maybebar[1]{\accentset{(-)}{#1}}

\newcommand{\longpage}{\enlargethispage{\baselineskip}}
\newcommand{\shortpage}{\enlargethispage{-\baselineskip}}


%\newcommand{\bd}{\ensuremath{\textrm{B}_\textrm{d}}}


\newcommand{\ftsigO}{\ensuremath{f_{\text{t},1}^\text{sig}}}
\newcommand{\ftsigI}{\ensuremath{f_{\text{t},2}^\text{sig}}}
\newcommand{\tsigO}{\ensuremath{\sigma_{\text{t},1}^\text{sig}}}
\newcommand{\tsigI}{\ensuremath{\sigma_{\text{t},2}^\text{sig}}}
\newcommand{\tsigII}{\ensuremath{\sigma_{\text{t},3}^\text{sig}}}

\newcommand{\Dzero}{D{\O}}
\def\BdToDstmunu  {\decay{\Bz}{\Dstarm \mup \neum}\xspace}


==> listsymbols <==
#!/bin/env python
import re

class TableWrite:
    """Write tables with correct header and footer"""
    
    def __init__(self,file):
        self.f = file
        self.columncount = 0
        self.tableopen= False
        self.tablebegin = r'\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l@{\extracolsep{\fill}}l@{\extracolsep{0.5cm}}l}'+'\n'
        self.tableend=r'\end{tabular*}'+'\n'

    def item(self,text):
        if not self.tableopen:
            self.f.write(self.tablebegin)
            self.tableopen=True
            self.columncount = 0
        self.f.write(text)
        if self.columncount<2:
            self.f.write(' & ')
            self.columncount+=1
        else:
            self.f.write(r' \\'+'\n')
            self.columncount=0

    def finish(self):
        if self.tableopen:
            if self.columncount>0:
                self.f.write(r' \\'+'\n')
            self.f.write(self.tableend+'\n')
            self.tableopen=False

    def header(self,text):
        self.finish()
        self.f.write(text+'\n')

fin = open('lhcb-symbols-def.tex')
outname = 'lhcb-symbols-list.tex'
fout = open(outname,'w')
print "All symbols are now available in the file %s." % outname

fout.write("""% This is an automatically generated appendix to template.tex. 
% When included it will show all the symbols defined in lhcb-symbols-def.tex.
%
% To regenerate with the latest definitions run the script ./listsymbols

\\section{List of all symbols}
""")

psection = re.compile(r'(%+)\s*(.*)')
pdef = re.compile(r'^\\def(\\.+?)[\s{]+[^%]*(%\s.+)*')
pnew = re.compile(r'^\\newcommand\{(\\\w+?)\}(\[\d\])*[\s\{]+[^%]*(%\s.+)*')
parg = re.compile(r'.+(#\d)+.*')

writer=TableWrite(fout)

for l in fin.readlines():

    # Match on section headers
    m = psection.match(l)
    if m:
        length = len(m.group(1))
        if length<=2:
            if length==1:
                writer.header('\\subsection{%s}' % m.group(2))
            else:
                writer.header('\\subsubsection{%s}' % m.group(2))

    # Match on the \def lines
    m = pdef.match(l)
    if m:
        marg = parg.match(m.group(1))
        if not marg:
            writer.item('\\texttt{\\textbackslash %s} & %s' 
                        % (m.group(1)[1:],m.group(1)))
        else:
            if m.group(2):
                pat1 = re.compile(r'#')
                pat2 = re.compile(r'(#\d)+')
                generic = re.sub(pat1,r'\#',m.group(1))
                example = re.sub(pat2,m.group(2)[2:],m.group(1))
                writer.item('\\texttt{\\textbackslash %s ' % generic[1:] +
                            '\\textbackslash %s} & %s' 
                            % (example[1:],example))
            else:
                print 'Ignoring line: %s' % l[:-1]

    # Match on the \newcommand lines
    m = pnew.match(l)
    if m:
        if not m.group(2):
            writer.item('\\texttt{\\textbackslash %s} & %s' 
                        % (m.group(1)[1:],m.group(1)))
        elif m.group(3):
            generic = str(m.group(3)[2:]).replace('{',r'\{').replace('}',r'\}')
            writer.item('\\texttt{\\textbackslash %s%s ' % 
                       (m.group(1)[1:],m.group(2)) +
                        '\\textbackslash %s%s} & %s%s' 
                        % (m.group(1)[1:],generic,
                           m.group(1),m.group(3)[2:]))
        else:
            print 'Ignoring line: %s' % l[:-1]
            
writer.finish()

fin.close()
fout.close()

